GitRanking: A Ranking of GitHub Topics for Software Classification using Active Sampling

GitHub is the world's largest host of source code, with more than 150M repositories. However, most of these repositories are not labeled or inadequately so, making it harder for users to find relevant projects. There have been various proposals for software application domain classification over the past years. However, these approaches lack a well-defined taxonomy that is hierarchical, grounded in a knowledge base, and free of irrelevant terms. This work proposes GitRanking, a framework for creating a classification ranked into discrete levels based on how general or specific their meaning is. We collected 121K topics from GitHub and considered $60\%$ of the most frequent ones for the ranking. GitRanking 1) uses active sampling to ensure a minimal number of required annotations; and 2) links each topic to Wikidata, reducing ambiguities and improving the reusability of the taxonomy. Our results show that developers, when annotating their projects, avoid using terms with a high degree of specificity. This makes the finding and discovery of their projects more challenging for other users. Furthermore, we show that GitRanking can effectively rank terms according to their general or specific meaning. This ranking would be an essential asset for developers to build upon, allowing them to complement their annotations with more precise topics. Finally, we show that GitRanking is a dynamically extensible method: it can currently accept further terms to be ranked with a minimum number of annotations ($\sim$ 15). This paper is the first collective attempt to build a ground-up taxonomy of software domains.

==> src/Study.tex <==
\CDS{Da revisionare}
In their recent work about multi-classification of \GH projects, Izadi \etal \citep{izadi2020topic} compare different multi-label classifier to recommend \GH topics.

\subsection{Dataset Description}
To enable the ASAP algorithm, we used the Repologue dataset composed of 135,489 repositories.
\subsection{Crawling phase}
\subsection{Mining rules}
\SC{Stiamo cercando di fare una lista piu automatica, quindi magari aspettiamo a espandere questa sezione}
To reduce unrelevant topics, Repologue makes use of several hand-written mining rules. They have been manually defined by building direct relationships among the terms. For instance, topics \emph{firefox} and \emph{chrome} are mapped to the unique term \emph{browser}. Thus, we employ such rules to enhance the performances of our previous work by adapting some of them considering our dataset. Specifically, we perform the following preprocessing steps in other to aggregate topics:
\begin{itemize}
\item [--] Remove punctuation, digits, non-English and non-ASCII characters,
\item [--] Replace popular software engineering and computer science related abbreviations and acronyms such as lib, app, config, DB, doc, and env with their formal form in the dataset;
\item[--] Identify a list of most frequent and informative tokens;% such as lib and api from the list of all names and split tokens based on them. For instance, svmlib is split to two tokens of svm and lib,
\item[--] Remove abstract concepts such as emails, URLs, usernames, markdown symbols, code snippets, dates, and times to normalize the text using regular expressions;
\item [--] Split tokens based on several naming conventions including SnakeCase, camelCase, and underscores;
\item[--] Convert tokens to lower case;
\item [--] Omit stop words, then apply tokenization and lemmatization on the topics;
\item [--] Remove topics with a frequency of less than a given threshold. This omits uninformative and infrequent topics;
\end{itemize}



